Constraining Cosmology with Simulation-based inference and Optical Galaxy Cluster Abundance

We test the robustness of simulation-based inference (SBI) in the context of cosmological parameter estimation from galaxy cluster counts and masses in simulated optical datasets. We construct ``simulations'' using analytical models for the galaxy cluster halo mass function (HMF) and for the observed richness (number of observed member galaxies) to train and test the SBI method. We compare the SBI parameter posterior samples to those from an MCMC analysis that uses the same analytical models to construct predictions of the observed data vector. The two methods exhibit comparable performance, with reliable constraints derived for the primary cosmological parameters, ($\Omega_m$ and $\sigma_8$), and richness-mass relation parameters. We also perform out-of-domain tests with observables constructed from galaxy cluster-sized halos in the Quijote simulations. Again, the SBI and MCMC results have comparable posteriors, with similar uncertainties and biases. Unsurprisingly, upon evaluating the SBI method on thousands of simulated data vectors that span the parameter space, SBI exhibits worsened posterior calibration metrics in the out-of-domain application. We note that such calibration tests with MCMC is less computationally feasible and highlight the potential use of SBI to stress-test limitations of analytical models, such as in the use for constructing models for inference with MCMC.

==> macros.tex <==
\DeclareRobustCommand{\VAN}[3]{#2}
\let\VANthebibliography\thebibliography
\def\thebibliography{\DeclareRobustCommand{\VAN}[3]{##3}\VANthebibliography}



==> packages.tex <==
\usepackage{newtxtext,newtxmath}

\usepackage[T1]{fontenc}
\usepackage{comment}

% Only include extra packages if you really need them. Common packages are:
\usepackage{graphicx}	% Including figure files
\usepackage{amsmath}	% Advanced maths commands
\usepackage{multicol}
% \usepackage{amssymb}	% Extra maths symbols

==> table_QuijoteTests.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
\begin{tabular}{| l | l |l|l|l|l|l|l|l|l|}
\hline
                               &                        & $\Omega_m$ & $\Omega_b$ & $h$ & $n_s$ & $\sigma_8$ & $M_\mathrm{A}$ & $M_\mathrm{B}$ & $\mathrm{ln} \sigma$ \\ \hline
\multirow{4}{*}{1} & Truth          & 0.1391 & 0.0618 & 0.7475 & 1.1545 & 0.8485 & 4.4351 & 1.4396 & 0.6555                   \\ \cline{2-10} 
                               & Qui-SBI & 0.1349$\pm$0.0023 & 0.0462$\pm$0.0079 & 0.7407$\pm$0.0820 & 1.0701$\pm$0.0585 & 0.8558$\pm$0.0067 & 4.4166$\pm$0.0153 & 1.4179$\pm$0.0343 & 0.6459$\pm$0.0126                      \\ \cline{2-10} 
                               & Ana-SBI & 0.1420$\pm$0.0027 & 0.0464$\pm$0.0085 & 0.7310$\pm$0.0882 & 1.0668$\pm$0.0595 & 0.8567$\pm$0.0057 & 4.4132$\pm$0.0160 & 1.4040$\pm$0.0350 & 0.6490$\pm$0.0129                     \\ \cline{2-10} 
                               & MCMC    &            &            &     &       &            &                &                &                      \\ \hline
\multirow{4}{*}{2} & Truth             & 0.3017 & 0.0386 & 0.6301 & 0.8745 & 0.9729 & 3.6096 & 1.2252 & 0.7056                      \\ \cline{2-10} 
                               & Qui-SBI & 0.3037$\pm$0.0027 & 0.0528$\pm$0.0089 & 0.6239$\pm$0.0618 & 0.8990$\pm$0.0487 & 0.9749$\pm$0.0046 & 3.5893$\pm$0.0099 & 1.2070$\pm$0.0208 & 0.7310$\pm$0.0104                     \\ \cline{2-10} 
                               & Ana-SBI & 0.3096$\pm$0.0056 & 0.0535$\pm$0.0092 & 0.6402$\pm$0.0745 & 0.9036$\pm$0.0587 & 0.9773$\pm$0.0072 & 3.6089$\pm$0.0122 & 1.2254$\pm$0.0231 & 0.7152$\pm$0.0133                      \\ \cline{2-10} 
                               & MCMC    &            &            &     &       &            &                &                &                      \\ \hline
\multirow{4}{*}{ 3} & Truth           & 0.1763 & 0.0576 & 0.7071 & 0.9759 & 0.7607 & 3.2155 & 1.0004 & 0.5611                      \\ \cline{2-10} 
                               & Qui-SBI & 0.1719$\pm$0.0072 & 0.0550$\pm$0.0084 & 0.6220$\pm$0.0683 & 0.9318$\pm$0.0621 & 0.7667$\pm$0.0142 & 3.2823$\pm$0.0348 & 1.0624$\pm$0.0412 & 0.5370$\pm$0.0311                      \\ \cline{2-10} 
                               & Ana-SBI & 0.1768$\pm$0.0084 & 0.0528$\pm$0.0090 & 0.6585$\pm$0.0905 & 0.9383$\pm$0.0771 & 0.7790$\pm$0.0144 & 3.2811$\pm$0.0337 & 1.0751$\pm$0.0467 & 0.5274$\pm$0.0273                      \\ \cline{2-10} 
                               & MCMC    &            &            &     &       &            &                &                &                      \\ \hline
\multirow{4}{*}{4} & Truth            & 0.4947 & 0.0578 & 0.5393 & 0.8579 & 0.9799 & 3.3824 & 1.2464 & 0.5524                      \\ \cline{2-10} 
                               & Qui-SBI & 0.4858$\pm$0.0039 & 0.0526$\pm$0.0090 & 0.5519$\pm$0.0287 & 0.8426$\pm$0.0257 & 0.9842$\pm$0.0046 & 3.3855$\pm$0.0095 & 1.2506$\pm$0.0138 & 0.5513$\pm$0.0140                      \\ \cline{2-10} 
                               & Ana-SBI & 0.4794$\pm$0.0057 & 0.0533$\pm$0.0093 & 0.5753$\pm$0.0449 & 0.8645$\pm$0.0416 & 0.9945$\pm$0.0042 & 3.3943$\pm$0.0105 & 1.2394$\pm$0.0165 & 0.5420$\pm$0.0174                      \\ \cline{2-10} 
                               & MCMC    &            &            &     &       &            &                &                &                      \\ \hline
\multirow{4}{*}{5} & Truth           & 0.1839 & 0.0471 & 0.8675 & 1.0421 & 0.6845 & 4.7303 & 1.2298 & 0.7227                      \\ \cline{2-10} 
                               & Qui-SBI  & 0.1845$\pm$0.0032 & 0.0452$\pm$0.0077 & 0.7623$\pm$0.0742 & 1.1105$\pm$0.0470 & 0.6851$\pm$0.0051 & 4.6963$\pm$0.0272 & 1.1993$\pm$0.0459 & 0.7138$\pm$0.0128                      \\ \cline{2-10} 
                               & Ana-SBI & 0.1904$\pm$0.0033 & 0.0459$\pm$0.0086 & 0.7538$\pm$0.0823 & 1.1034$\pm$0.0557 & 0.6884$\pm$0.0042 & 4.6939$\pm$0.0295 & 1.1786$\pm$0.0634 & 0.7178$\pm$0.0126                      \\ \cline{2-10} 
                               & MCMC    &            &            &     &       &            &                &                &                      \\ \hline
\end{tabular}
\caption{\label{tbl:5Tests} 
Inference of eight parameters with three models on five test data sets. 
The test sets are differentiated by the truth value of each parameter. 
For each test, there are true parameters, parameter inferences from SBI on Quijote data, from SBI on Analytically produced data, and from MCMC on Quijote data.
}
\end{table*}
